Privacy Risks in Reinforcement Learning for Household Robots

The prominence of embodied Artificial Intelligence (AI), which empowers robots to navigate, perceive, and engage within virtual environments, has attracted significant attention, owing to the remarkable advances in computer vision and large language models. Privacy emerges as a pivotal concern within the realm of embodied AI, as the robot accesses substantial personal information. However, the issue of privacy leakage in embodied AI tasks, particularly concerning reinforcement learning algorithms, has not received adequate consideration in research. This paper aims to address this gap by proposing an attack on the training process of the value-based algorithm and the gradient-based algorithm, utilizing gradient inversion to reconstruct states, actions, and supervisory signals. The choice of using gradients for the attack is motivated by the fact that commonly employed federated learning techniques solely utilize gradients computed based on private user data to optimize models, without storing or transmitting the data to public servers. Nevertheless, these gradients contain sufficient information to potentially expose private data. To validate our approach, we conducted experiments on the AI2THOR simulator and evaluated our algorithm on active perception, a prevalent task in embodied AI. The experimental results demonstrate the effectiveness of our method in successfully reconstructing all information from the data in 120 room layouts. Check our website for videos.

==> backup.tex <==
%% reason for separate reconstruct of vector and image
{\color{red}based on the following reasons. 
First, the gradient inversion of linear layers is easier than convolution layers \cite{geiping2020inverting,zhu2020r-gap} because (1) linear layers contain more parameters than convolution layers; (2) linear layers have corresponding parameter element for each (input, output) element pair, while in convolution layers, each parameter element contributes to the calculation of multiple input and output elements, resulting in less effective updates of the reconstruction.
%The aggregation exacerbates the challenge as different samples may have the same aggregated results.
Second, we observe that features from the vector and visual input are usually combined in the vector form, enabling the neglect of convolution layers during the vector state reconstruction.
Third, as the error in the vector state reconstruction results in the accuracy drop in image reconstruction, an accurately reconstructed vector state obtained before the image state reconstruction is beneficial. %critical.


%%% adaptive lambda
Since $\lambda_i$ and $\lambda_d$ are critical to the effect of two terms in $L_{img}$, we use an adaptive weight as
%In addition to constant $\lambda$, we investigate floating weights of the gradient matching loss and TV loss, where the final gradient 
\begin{align}
    \lambda_i = \frac{\left\| {\partial L(g^{rec},g)}/{\partial s^{rec}_i} \right\|}{\left\|{\partial \text{TV}(s^{rec}_i)}/{\partial s^{rec}_i}\right\|}.
\label{equ:floating_lambda}
\end{align}
%adding the 2 loss functions, we also investigate the effect of balancing their effect by adjusting the gradient.
%The backpropagations of gradient matching loss and the TV loss are executed separately.
%The final gradient used to update $s^{rec}_i$ is
%\begin{align}
%    \Delta s^{rec}_i = \frac{\frac{\partial L(g^{rec},g)}{\partial s^{rec}_i}}{\left\| \frac{\partial L(g^{rec},g)}{\partial s^{rec}_i} \right\|} 
%    + \frac{\frac{\partial \text{TV}(s^{rec}_i)}{\partial s^{rec}_i}}{\left\|\frac{\partial \text{TV}(s^{rec}_i)}{\partial s^{rec}_i}\right\|}.
%\end{align}
%The gradient of the RGB image $s^{rec}_i$ and the depth image $s^{rec}_d$ undergo the same procedure.
The weight $\lambda_i$ in (\ref{equ:floating_lambda}) is then used in the gradient descent optimization of $s^{rec}_i$ with the gradient
\begin{align}
    \Delta s^{rec}_i = \frac{\partial L(g^{rec},g)}{\partial s^{rec}_i}
    + \lambda_i \frac{\partial \text{TV}(s^{rec}_i)}{\partial s^{rec}_i}.
\label{equ:update_image}
\end{align}
For updating $s^{rec}_d$, we use the same rule to adjust $\lambda_d$.


\begin{align}
    \left\| \hat{Q}-Q \right\|^{rec} \gets \left\| \hat{Q}^{rec} - \tilde{Q} \right\| \frac{\|g\|}{\|g^{rec}\|}.
\end{align}


\begin{table}[t]
    \centering
    \caption{IoU of coordinates for QGI and RGI.}
    \scalebox{.7}{
    \begin{tabular}{cc|ccccc}
        \toprule
         &  & bathroom & bedroom & kitchen & living room & average \\
        \midrule
        QGI & S1 & $0.933\pm0.169$ & $0.872\pm0.229$ & $0.949\pm0.133$ & $0.894\pm0.212$ & $0.912\pm0.192$ \\
        QGI & S2 & $0.995\pm0.028$ & $0.970\pm0.147$ & $0.911\pm0.264$ & $0.887\pm0.296$ & $0.941\pm0.217$ \\
        RGI & S1 & $1.000\pm0.000$ & $0.983\pm0.128$ & $1.000\pm0.000$ & $0.983\pm0.128$ & $0.992 \pm 0.091$ \\
        RGI & S2 & $1.000\pm0.000$ & $0.983\pm0.128$ & $1.000\pm0.000$ & $0.983\pm0.128$ & $0.992 \pm 0.091$ \\
        \bottomrule
    \end{tabular}}
    \label{tab:coord}
    \vspace{-4mm}
\end{table}


\begin{table}[t]
    \centering
    \caption{Percentage error (\%) in QGI.}
    \scalebox{.7}{
    \begin{tabular}{cc|ccccc}
        \toprule
        Setting & Metric & bathroom & bedroom & kitchen & living room & average \\
        \midrule
        \multirow{2}{*}{S1} & $\epsilon(\hat{Q})$ & $0.95\pm1.70$ & $1.35\pm1.61$ & $0.64\pm1.10$ & $1.19\pm1.76$ & $1.03\pm1.59$ \\
        & $\epsilon(Q)$ & $0.51\pm0.97$ & $0.89\pm1.61$ & $0.40\pm1.03$ & $0.40\pm1.03$ & $0.67\pm1.47$ \\
        \midrule
        \multirow{2}{*}{S2} & $\epsilon(\hat{Q})$ & $0.11\pm0.16$ & $0.34\pm0.62$ & $0.45\pm1.24$ & $1.01\pm2.54$ & $0.48\pm1.49$ \\
        & $\epsilon(Q)$ & $0.11\pm0.24$ & $0.16\pm0.30$ & $0.25\pm0.78$ & $0.65\pm0.24$ & $0.29\pm1.29$ \\
        %& $Q$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
        \bottomrule
    \end{tabular}}
    \label{tab:qvalues}
    \vspace{-4mm}
\end{table}



histogram of IoU, Q-value and Target Q-value
\begin{wfigure}{r}{0.35\textwidth}
    \vspace{-5mm}
    \centering
    \includegraphics[width=0.35\textwidth]{images/dqn_initialnetwork_rgbdepthcoord_stateactionqvaluesrecover_ReLU_wisebalance_hist.jpg}
    \vspace{-7mm}
    \caption{Histogram of coordinate IoU, percentage error of Q-values and target Q-values.}
    \vspace{-8mm}
    \label{fig:hist}
\end{wrapfigure}


%%% multimodal input state reconstruction: abalation study -- joint vs separate
\begin{table}[b]
    \centering
    \caption{Comparison of Joint QGI and QGI.}
    \scalebox{.6}{
    \begin{tabular}{c|ccccc}
        \toprule
        Method & PSNR/SSIM (RGB) $\uparrow$ & PSNR/SSIM (depth) $\uparrow$ & IoU $\uparrow$ & $\epsilon(\hat{Q})$(\%) $\downarrow$ & $\epsilon(Q)$(\%) $\downarrow$ \\
        \midrule
        %Joint & $19.02\pm5.71$/$0.655\pm0.183$ & $19.63\pm5.76$/$0.666\pm0.144$ & $0.057\pm0.151$ & $45.97\pm11.75$ & $27.18\pm37.56$ \\ 
        Joint QGI & $19.0\pm5.7$/$0.66\pm0.18$ & $20.3\pm7.6$/$0.67\pm0.19$ & $0.057\pm0.151$ & $46.0\pm11.8$ & $27.2\pm37.6$ \\ 
        %Ours & $21.77$/$0.747$ & $22.13$/$0.703$ & $0.912\pm0.192$ & $1.03\pm1.59$ & $0.67\pm1.47$ \\
        QGI & $21.8\pm3.9$/$0.74\pm0.10$ & $24.4\pm4.2$/$0.76\pm0.11$ & $0.912\pm0.192$ & $1.03\pm1.59$ & $0.67\pm1.47$ \\
        %Ours & $21.77\pm3.87$/$0.747\pm0.095$ & $22.13\pm4.53$/$0.703\pm0.135$ & $0.912\pm0.192$ & $1.03\pm1.59$ & $0.67\pm1.47$ \\
        \bottomrule
    \end{tabular}}
    \label{tab:ablation joint vs step}
\end{table}




\begin{table*}[!t]
    \centering
    \caption{PSNR $(\uparrow)$ and SSIM $(\uparrow)$ of the RGB and depth images.}
    \scalebox{1}{
    \begin{tabular}{ccc|c|cccccccc}
        \toprule
        method & setting & State & Metric & bathroom & bedroom & kitchen & living room & average & best  \\
        \midrule
        \multirow{4}{*}{QGI} & \multirow{4}{*}{S1} & \multirow{2}{*}{RGB} & PSNR & $22.81\pm5.99$ & $19.73\pm5.16$ & $21.41\pm5.69$ & $20.11\pm6.17$ & $21.02\pm5.86$ & 32.17\\
        & & & SSIM & $0.761\pm0.141$ & $0.735\pm0.146$ & $0.724\pm0.167$ & $0.696\pm0.170$ & $0.729\pm0.157$ & 0.929 \\
        & & \multirow{2}{*}{depth} & PSNR & $24.89\pm10.43$ & $22.85\pm7.42$ & $23.26\pm7.17$ & $21.72\pm7.05$ & $23.18\pm8.17$ & 38.09 \\
        & & & SSIM & $0.809\pm0.249$ & $0.823\pm0.161$ & $0.803\pm0.197$ & $0.793\pm0.162$ & $0.807\pm0.195$ & 0.983 \\
        \midrule
        \multirow{2}{*}{QGI} & \multirow{2}{*}{S2} & \multirow{2}{*}{depth} & PSNR & $29.78\pm7.33$ & $26.14\pm7.67$ & $26.45\pm7.27$ & $23.49\pm7.29$ & $26.46\pm7.68$ & 45.76 \\
        & & & SSIM & $0.930\pm0.111$ & $0.899\pm0.152$ &$0.918\pm0.092$ & $0.894\pm0.129$ & $0.910\pm0.123$ & 0.994 \\
        \midrule
        \multirow{4}{*}{RGI} & \multirow{4}{*}{S1} & \multirow{2}{*}{RGB} & PSNR & $18.03\pm5.76$ & $16.98\pm5.93$ & $17.65\pm4.85$ & $15.84\pm4.60$ & $17.12\pm5.35$ & 31.20 \\
        & & & SSIM & $0.564\pm0.190$ & $0.550\pm0.186$ & $0.551\pm0.166$ & $0.511\pm0.163$ & $0.544\pm0.176$ & 0.924 \\
        & & \multirow{2}{*}{depth} & PSNR & $19.75\pm6.66$ & $18.80\pm6.26$ & $18.71\pm5.35$ & $17.04\pm5.17$ & $18.58\pm5.94$ & 36.41 \\
        & & & SSIM & $0.582\pm0.197$ & $0.590\pm0.164$ & $0.594\pm0.158$ & $0.559\pm0.141$ & $0.581\pm0.166$ & 0.940 \\
        \midrule
        \multirow{2}{*}{RGI} & \multirow{2}{*}{S2} & \multirow{2}{*}{depth} & PSNR & $39.19\pm5.34$ & $37.87\pm3.57$ & $36.91\pm4.31$ & $34.85\pm4.99$ & $37.21\pm4.84$ & $58.83$ \\
        & & & SSIM & $0.972\pm0.018$ & $0.968\pm0.018$ & $0.963\pm0.022$ & $0.953\pm0.024$ & $0.964\pm0.022$ & $1.000$ \\
        \bottomrule
    \end{tabular}}
    \label{tab:psnr-ssim}
    \vspace{-4mm}
\end{table*}


\begin{table}[t]
    \centering
    \caption{IoU, Percentage Error and Absolute Error.}
    \scalebox{.92}{
    \begin{tabular}{c|ccccc}
        \toprule
         & IoU $(\uparrow)$ & $\epsilon(\hat{Q})$ (\%) $(\downarrow)$ & $\epsilon(Q)$ (\%) $(\downarrow)$ & err$(r)$ $(\downarrow)$ \\
        \midrule
        QGI S1 & $0.912\pm0.192$ & $1.03\pm1.59$  & $0.67\pm1.47$ & - \\
        QGI S2 & $0.941\pm0.217$  & $0.48\pm1.49$ & $0.29\pm1.29$ & - \\
        \midrule
        RGI S1 & $0.992 \pm 0.091$ & - & - & 1.6e-8$\pm$3.4e-8\\
        RGI S2 & $0.992 \pm 0.091$ & - & - & 2.1e-8$\pm$3.5e-8 \\
        \bottomrule
    \end{tabular}}
    \label{tab:coord qvalue reward}
\end{table}

==> reviews.tex <==
\section{Comments from reviewers}

Dates to keep in mind: \\ \\
Feb 6: Paperplaza opens for Final paper submission \\
March 6: Final paper submissions due \\
March 6: Author registration due \\
April 12: Presentation video and Graphical Abstract due \\
May 13-May 17: ICRA!\\


TODOs:
\begin{itemize}
    \item \textbf{not super related to robotics}: both paper written and experiment
    \item \textbf{not enough experiment settings}: more RL model, more training stages, larger batch size, more tasks, more modal, and using physical robots
    \item \textbf{more explanation}: 1) cosine similarity, make it clear why using a loss function from another paper; 2) comparison between our method and those baselines
    \item \textbf{more explanation}: 1) gradient calculation; 2) victim model; 3) robustness, effectiveness, whether it can transfer to other cases
\end{itemize}


\subsection{ 38051} 	This paper presents a relevant problem in robotics, specifically, the data leak by gradients in distributed robot systems trained within the federated learning framework. This paper proposes a gradient inversion method for reinforcement learning algorithms, including REINFORCE and Deep Q-learning, that uses gradients to recover the image state, action, reward, and Q-values. Results show that this approach shows good performance in reconstructing indoor images in datasets, which indicates its ability to steal data from users' houses through gradient transmission in federated learning. 
Strengths:

1. The supplementary video is quite clear and covers sufficient experiment results including the simulation environment dataset, real-world dataset and RL simulator, and reconstructed RGB and depth images.  

2. The theoretical parts in this paper are quite solid and detailed and helpful to understand the algorithm proposed.  

3. The figures used in this paper are very clear in illustrating the approach proposed.  

Weaknesses:

1. This paper mentioned large fundamental models in the abstract and the introduction, but the overall problem is set under a federated learning framework, so I think it might be better to remove these irrelevant contents or elaborate on this part by justifying its relevance to the main topic. 

2. In the result and discussion part, the author should address the following two points to give some insights about the experimental results given in Table 1. (1) Why does the reconstruction quality of QGI and RGI differ a lot, both in PSNR and SSIM? (2) Why is the reconstruction quality of the depth image in both methods so high? Properly addressing both points helps readers to understand this paper's contribution and the problem it raises. 

3. More experiments on real robots should be included. This paper mostly applies a research problem found in the federated learning domain to robotics, but evidence for the importance of this problem in robotics or experiments on real robot systems using federated learning is not included. Solid evidence of its application in real-world robotics will help readers understand the meaning and importance of this problem in the robotics community. 

TODOS:
\begin{itemize}
    \item Fundamental models: modify abs and intro to justify the relevance to the main topic
    \item explanation of experiment: why results of QGI and RGI differ a lot in results
    \item add experiment: real robot experiment using a federated learning framework -- ask changyi or William for help
\end{itemize}

\subsection{ 38053 }	The paper introduces a novel approach to tackle the multi-modal data reconstruction problem from the gradient of reinforcement learning (RL), demonstrating that information leaking is a critical concern in RL. Specifically, The author presents a novel gradient inversion technique applicable to both value-based and gradient-based RL, aiming to reconstruct multi-modal input information encompassing states, actions, and supervision signals within RL. A cosine similarity loss is adopted to reconstruct multi-modal states in conjunction with the total variation loss, serving as a penalty for noise patterns based on the gradients of the true and reconstructed data. To obtain a gradient from constructed training data in R.L., the author calculates the reconstructed gradient from the error direction instead of obtaining it from the original objective function, allowing rule-based methods to reconstruct action and supervision signals efficiently. Finally, experimental results conducted on the AI2THOR simulator and active perception task validate the effectiveness of the proposed gradient inversion approach in reconstructing multi-modal data in the value-based and the gradient-based R.L. algorithm.  

Strengths:
Overall, the paper addresses an interesting subject with extensive experimental results. The organization of the paper is clear, and the presentation of the technical details is consistent and easy to follow. I appreciate the discussion part in their conclusion to show the limitation of this work. There are some comments from this reviewer.

1. The topic of this paper is more related to data privacy rather than robotics. Still, it's a decent conference paper. It would be beneficial for the authors to clarify their contribution to the field of robotics and automation.

2. The authors employ a cosine similarity loss to reconstruct multi-modal states, which bears a strong resemblance to the equation (4) found in a related work on general optimization-based attack approaches. Can the authors elaborate on the differences between the two?(Reference: "Geiping J, Bauermeister H, Dröge H, et al.Inverting gradients-how easy is it to break privacy infederated learning? Advances in Neural InformationProcessing Systems, 2020, 33: 16937-16947")

3. In Section V.A., I recommend adding a table to present the qualitative results in the "State: Coordinate" part.

4. Regarding the references, Please ensure that the references are formatted consistently throughout the paper.This includes capitalizing the titles of conferences andjournals (e.g., 'Advances in neural information processing systems' should be 'Advances in Neural Information Processing Systems'). Additionally, please standardize theuse of abbreviations for conference names and ensure thatall references consistently include page numbers. Overall, the paper addresses an important issue andprovides valuable insights, but it needs further clarityregarding its relevance to robotics.

TODOs:
\begin{itemize}
    \item clarify the contribution to the field of robotics
    \item clarify of the novelty: this work uses the same cosine similarity loss as the previous work inverting-gradient
    \item modify result representation: add a table of quantitative results for scalar and vector data
    \item reference format: check the format inside the bib file, especially the use of capital letters
\end{itemize}

\subsection{ 38057} 	The paper presents a novel method that exploits gradient inversion to recreate private information such as states, actions, and supervision signals from value-based and gradient-based RL algorithms. These algorithms often use gradients derived from user data, which, although not directly shared, can inadvertently reveal sensitive information. The paper's proposed attack highlights a significant vulnerability in federated learning frameworks, where gradients are the only shared information. To demonstrate the feasibility of this attack, the authors performed experiments within the AI2THOR simulator, focusing on active perception tasks in embodied AI. Their results show that the method can effectively reconstruct complete information from the gradients across various scenarios. In general, the paper is novel and well-written. More detailed comments are listed as follows.

Strengths:
1. This paper systematically introduces the concept of gradient inversion and proposes corresponding methods in the settings of reinforcement learning and robotic visual navigation. The idea and tasks are novel and make sense to me.
2. The paper investigates the robotic task based on multimodal data, including the depth image, the RGB image, and the coordinate of the targeted object in the scene. This is a significant departure from previous works that have largely focused on unimodal data type, e.g., RGB images.
3. This work investigates the possibility of revealing private state, action, and Q-values from gradients in the settings of reinforcement learning, with a combination of optimization-based and rule-based method.
4. The paper proposes a that method that provides comprehensive analysis covering both implementations designed for on-policy and off-policy RL algorithms.
5. The proposed method interprets the gradient as the result of backpropagation from an error direction other than from the objective function, thus circumventing relying on the RL objective function, making it applicable to various RL algorithms.

Weaknesses
1. The experiments were conducted on the initialized networks with a relatively simple network structure, which may not provide a comprehensive understanding of the method's effectiveness across different stages of learning and more advanced applications in robotic tasks. It is understandable as it is the first work of its kind for RL and robotics, while it would be beneficial to discuss this limitation in the paper.
2. It would be helpful to provide more insights on how the proposed method could handle and take advantage of sequential inputs, as demonstrated in the attached video. Would it be possible to implement sequential state reconstruction instead of a single-step calculation? Would this improve the quality of reconstruction?
3. It would be more helpful to discuss the limitation of the surrogate objective of the optimization-based gradient inversion. Specifically, how would the error direction change if the default batch size and last layer of the neural network are specified? 
4. The proposed method and baselines are evaluated on different scenarios of visual navigation tasks. It would be beneficial to discuss its generalizability to other tasks.

TODOs
\begin{itemize}
    \item The experiments are done with init network, what about others
    \item sequential reconstruction
    \item limitation of the surrogate gradient calculation method
    \item what about other tasks -- no privacy issues, so no
\end{itemize}


\subsection{ 38061}	This groundbreaking study is the first of its kind to propose a Gradient Inversion Attack strategy specifically tailored for federated reinforcement learning. The researchers have successfully developed two innovative pipelines, namely QGI and RGI, which are designed to reconstruct multimodal data. This research stands out due to its enlightening and pioneering nature, particularly in addressing the potential risk of information leakage within reinforcement learning, an issue that, to my knowledge, has never been previously discussed. The practicability of the Gradient Inversion Attack approach is further endorsed by experiments conducted using a simulation.

However, I must express a few reservations pertaining to this work:

1.While the paper meticulously explains the process of Gradient Inversion, it unfortunately overlooks the critical aspect of gradient computation. Although this omission might be due to constraints with respect to length, inclusion of such details would undoubtedly make the discussion more comprehensive.
2.The experimental component of the paper effectively demonstrates the capability of Gradient Inversion in terms of reconstruction. However, the paper could significantly improve by broadening its scope to include comparisons between different reinforcement learning models and also between models at varying stages of training, thereby providing deeper insights into the reconstruction efficacy.

In summary, this research is characterized by clarity in both thought and language, making it an insightful contribution to the field. Nevertheless, taking into account the aforementioned points would considerably
enhance the overall impact and comprehensibility of this work. 

TODOs:
\begin{itemize}
    \item Not sure what: include discussion of the gradient computation: what gradient computation?
    \item More experiments: different RL models, different stages
\end{itemize}


\subsection{ 38063} Comment:
1. This paper has complete structure, clear logic and sufficient simulation results. 
2. While the background is fascinating and important, there should be more description about applying gradient inversion techniques to RL. 
3. More description about comparison with related algorithms should be added. 
4. The proposed problem is novel and meaningful, and there are indeed problems existing in the background introduction. 
The original image information can be reconstructed using gradient, and the experimental results also prove the effectiveness of the reconstruction algorithm. Looking forward to better work 

TODOS:
\begin{itemize}
    \item writing: less about background, more about applying GI to RL
    \item writing: more description about baselines and comparison
\end{itemize}

\subsection{ 38065 }	In general, this paper delves into a relatively underexplored area, namely, the privacy leakage risks within reinforcement learning. The paper introduces gradient reversal attack methods tailored for DQN and REINFORCE algorithms, validated within the AI2THOR simulation environment. The work exhibits a certain degree of innovation, marking the initial foray into privacy attacks within the realm of reinforcement learning. The central contribution of the paper lies in the proposal of a multi-modal input reconstruction pipeline, incorporating rule-based methods for reconstructing actions and supervisory signals. Experimental results demonstrate the successful reconstruction of states, actions, and reward signals, underscoring the potential for privacy leakage solely from shared gradient information. However, several areas for improvement warrant consideration.

Comments 1:
The experimental setup employed a relatively simple environment (AI2THOR). It remains an open question whether the algorithm's reconstruction performance would be affected when operating in more complex environments. Further investigation is needed to assess the algorithm's robustness and effectiveness in scenarios with increased environmental complexity.

Comments 2:
The proposed attack method in the paper is currently designed for a batch size of 1. It is unclear how the method would behave with larger batch sizes, as the dynamics of the algorithm might significantly change.
Whether the algorithm can be extended to handle larger batch sizes remains an open question and an area for potential future research. 

Comments 3:
The recognizability of the reconstructed images in the paper is relatively limited. In the future, it would be beneficial to consider providing additional quantitative or qualitative analyses to substantiate that the reconstructed content indeed reflects private information from the real environment.

Comments 4:
The paper primarily focuses on the reconstruction of visual inputs, but whether other types of inputs in reinforcement learning, such as voice commands or textual information, also entail similar privacy leakage risks remains an unexplored area in need of further research.

TODOs:
\begin{itemize}
    \item robustness and effectiveness in more complex environment: AI2THOR is too simple
    \item batch size: what would happen when batch size is larger
    \item add experiment results from real environments
    \item other modal: this one focuses on visual input, how about voice commands and textual info
\end{itemize}


\subsection{ 38075} 	The paper presents a gradient inversion methodology for deep reinforcement learning, specifically for DQN and REINFORCE algorithms. The authors claim that QGI and RGI are the first frameworks to investigate the privacy leakage problem by recovering data in RL from gradient information. The key contribution is their design of novel pipelines to reconstruct multimodal state data, such as RGB and depth images, discrete actions, and supervision reward signals. The authors validate their approach in AI2THOR, an open-source interactive environment for embodied AI. The reviewer is impressed that the authors are the first to reconstruct multimodal data, as well as actions and rewards in the DRL field.

The comments for this paper are as follows:

1. There is a concern as to why the paper did not address action selection strategy in its action reconstruction methodology. Action selection is critical in Deep Reinforcement Learning (DRL), particularly for exploration-exploitation balance, notably in the Deep Q-Network (DQN) algorithm, where an epsilon-greedy strategy commonly dictates random actions, irrespective of Q-values.
However, the paper does not clarify if the victim model utilizes this strategy or if it simply selects actions based on Q-values, nor does it propose a method to handle such strategies. Action selection is a cornerstone in DRL, universally applied across most DRL methods, including DQN. The authors distinguish their work from other gradient inversion studies by focusing on reconstructing multimodal states, actions, and rewards in DRL. For this claim to hold, the recovery process must accommodate DRL's distinctive elements, like random actions. The reviewer suggests that the authors should develop a pipeline that incorporates the widely used action selection strategy in DRL or acknowledge its absence as a limitation.

2. The paper omits details about the victim model, which complicates assessing the presented gradient inversion challenges. The authors cite the paper [11], which suggests that the training level of the victim network can influence the attacker's reconstruction quality. It is pointed out that for well-trained networks, the loss function's gradient might approach zero, eliminating the possibility of extracting distinct features. This issue is relevant to DRL problems as well. Despite the 6-page limit, an explanation of the model's network, which the gradient inversion attack targets, is essential. Additionally, there is no network explanation regarding the reconstruction of images and vector states. While there is a description of the objective function, there is no explanation for the network used for RGB and depth image reconstruction. This omission hinders the reproducibility of this work. If this detail was omitted due to paper length limitations, one solution could be to separate this paper's two pipelines, QGI and RGI, and rewrite them as individual papers.

4. The authors stated in the manuscript, "When the batch size is larger than 2, the action reconstruction may require enumeration or optimization." From the reviewer's perspective, it seems that the action reconstruction constrains the batch size to a small number, but the reason for this is unclear, and justification is needed for the claim of novelty despite such a limitation.
5. The manuscript seems to disregard the impact of hyperparameters such as the learning rate. Since the learning rate can change the gradient's magnitude, it may affect the accuracy of gradient inversion. The reviewer wonders if this work presupposes complete access to the hyperparameter configuration of the victim network. It is important to address whether this assumption is widely accepted in the field of gradient inversion. 	 

TODOs:
\begin{itemize}
    \item 
\end{itemize}


\subsection{ 38077} 	This paper addresses the issue of privacy leakage in embodied AI tasks, specifically in reinforcement learning algorithms. The authors propose an attack using gradient inversion to reconstruct states, actions, and supervision signals. They utilize gradients computed based on private user data to optimize models, without storing or transmitting the data to public servers. These gradients contain enough information to potentially expose private data. The authors validate their approach through experiments on the AI2THOR simulator and demonstrate the effectiveness of their method in successfully reconstructing all information from the data across 120 room layouts.

The innovation of this paper lies in proposing a gradient inversion attack on reinforcement learning algorithms in the context of embodied AI tasks. The authors introduce two frameworks, QGI and RGI, to reconstruct multimodal information solely from the gradients shared by the RL algorithm. This approach addresses the privacy leakage issue in RL and highlights the potential risks associated with federated learning techniques. The authors also provide novel pipelines for reconstructing the different modal types of input data.

The weakness of this paper I think is authors claim the proposed method is a framework to investigate the information leaking problem by reconstructing data in RL from the gradient. However, the experimental is limited to reconstruction of an active perception task. The author did not explicitly mention whether the proposed method can be transferred to other RL problems easily. Furthermore, only deep Q learning and REINFORCE are discussed. There are many other deep RL algorithms such as PPO, DDPG, A2C. The paper would be more stronger if the author could discuss more about whether the proposed method can be also applied on these algorithms.

Overall, this paper provides valuable insights into the privacy risks associated with RL algorithms and offers a novel framework for addressing privacy leakage in embodied AI tasks. 	 


TODOs:
\begin{itemize}
    \item whether this can transfer to other problems, or only active perception
    \item whether this can transfer to other RL models, or only DQN and Reinforce
\end{itemize}
